ARMDN: Associative and Recurrent Mixture Density Networks for eRetail Demand Forecasting

Accurate demand forecasts can help on-line retail organizations better plan their supply-chain processes. The challenge, however, is the large number of associative factors that result in large, non-stationary shifts in demand, which traditional time series and regression approaches fail to model. In this paper, we propose a Neural Network architecture called AR-MDN, that simultaneously models associative factors, time-series trends and the variance in the demand. We first identify several causal features and use a combination of feature embeddings, MLP and LSTM to represent them. We then model the output density as a learned mixture of Gaussian distributions. The AR-MDN can be trained end-to-end without the need for additional supervision. We experiment on a dataset of an year's worth of data over tens-of-thousands of products from Flipkart. The proposed architecture yields a significant improvement in forecasting accuracy when compared with existing alternatives.

==> cubist.tex <==
\section{Boosted Cubist Models}
In this section we present the design of a non-deep learning based model that combines several ideas from traditional machine learning.that best suits our setup and task.

Cubist\cite{kuhn13}, an extension of Quinlan's M5 model \cite{quinlan92,quinlan93,quinlan93a}, is primarily a rule based method which uses a couple of innovations to improve the results further. %The Cubist model has gained in popularity  since its integration into R \cite{kuhn13} . 
Overall, a tree is generated, and based on the predictors used in the preceding splits, a linear regression model is executed at the terminal node. While the final prediction is based on the models of the terminal node, they are smoothed using a linear model at its preceding node. The process of smoothening appears recursively up the branches of the tree. In addition, the cubist model introduces two innovative approaches to further refine the predictions i) Ensembling with committees and ii) Nearest neighbor based adjustments. Both adjustments are independent of each other an can be used separately or in conjunction with each other. To incorporate features of the time-series a number of autoregressive features were used for each instance like lag of 1 day sale, lag of 1 week (mean) sale and lag of 1 month (mean sale) were used. Cubist was executed in a one-step ahead fashion where the for the $t^{th}$ time step in the future, the output from the $t-1^{th}$ time step was used as an input to calculate the lag features. Along with lag features, other time series features like week of year and time since first sale/launch were used as well. 

\subsubsection*{}{Ensembling with committees}
Cubist has the ability to use a sequence of model trees, an approach akin to boosting, called committees. After the first rule-based tree is generated, an iterative sequence of trees are generated such that the training set outcome is adjusted based on the fit of the prior tree, thereby building a new set of rules. Specifically, the $k^{th}$ committee model uses an adjusted response 
\begin{equation}
y_{i(k)}=2y_{i(k-1)} - \hat{y}_{i(k)}
\end{equation}
Once the full set of model trees have been created, new samples are predicted using every individual tree and the final prediction output is the mean of the prediction from the individual trees i.e. it finally produces an ensembled output.

\subsubsection*{}{Nearest neighbor based adjustments}
Other than the committees approach, Cubist also has the ability to adjust the predictions of the rule-based models using nearest neighbors within the training set. Once a model tree, with or without committees is generated, a sample is predicted by this model. Thereby Cubist finds the $k$ nearest neighbor of the predicted sample from the training set and uses an average of the $k$ training points to readjust the prediction. The final prediction is therefore given by 
\begin{equation}
\hat {y}=\frac{1}{k} \sum_{l=1}^kw_l[t_l+(\hat{y}-\hat{t}_l)]
\end{equation}
where $t_l$ is the observed outcome of training neighbor, $\hat{t}_l$ is the model prediction of the neighbor and $w_l$ is the weight calculated using the distance of the training set neighbors to the new sample.

